AttributionLab: Faithfulness of Feature Attribution Under Controllable Environments

Feature attribution explains neural network outputs by identifying relevant input features. The attribution has to be faithful, meaning that the attributed features must mirror the input features that influence the output. One recent trend to test faithfulness is to fit a model on designed data with known relevant features and then compare attributions with ground truth input features.This idea assumes that the model learns to use all and only these designed features, for which there is no guarantee. In this paper, we solve this issue by designing the network and manually setting its weights, along with designing data. The setup, AttributionLab, serves as a sanity check for faithfulness: If an attribution method is not faithful in a controlled environment, it can be unreliable in the wild. The environment is also a laboratory for controlled experiments by which we can analyze attribution methods and suggest improvements.

==> chapters/999-method-old.tex <==
\section{A transparent environment to obtain true attribution}\label{sec:method:transparent_env}
The incentive of this work is to establish an environment where we know which input features are relevant to the output of a model. This laboratory setup allows for gauging the faithfulness of feature attribution methods. We can identify which attributions are not aligned with the ground truth features of the network and understand the sources of failures. Prior to detailing the setup, we underline the necessity of designing both the \emph{data} and the \emph{network}.

To realize the controlled setup for evaluating explanations, one might design a dataset where the associations between input features and output labels are known: e.g., a simple dataset of squares and circles. Indeed, prior approaches~\citep{arras2022clevr,zhou2022feature,schuessler2021two4two,agarwal2023evaluating} design synthetic datasets and train a model on them. The underlying assumption is that a model learns the true labeling function once the model achieves peak performance on the synthetic dataset during the learning process. However, it is unclear whether the trained network uses the entire square, straight lines, or just corners to identify the square. How can we know if a network uses an entire square for decision-making in this setup? This phenomenon is considered as the Rashomom effect, which we rephrase in the following definition:
%
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/maintext/overview_sde.pdf}
    \caption{Overview of two synthetic environments. Single-color-modulo takes a monochromatic image as input and outputs the modulo $N$ result of the total number of white pixels. Multi-color-sum accepts colored input and returns an output score vector counting the number of pixels in each target color. The networks follow conventional neural network designs (having sufficient complexity for simulation purposes). The networks are explicitly programmed (the parameter values are set by us, not the optimization) to perform these tasks. Therefore, we know which input features are relevant to the network.
    % The example output numbers are made up for illustration purposes.
    Additional details on the model designs can be found in the Section~\ref{sec:method:design} and Appendix~\ref{sec:appendix:detail_model_design}.}
    \label{fig:synthetic_environment}
\end{figure}
\begin{figure}[b]
    \centering
    \includegraphics[width=0.8\columnwidth]{figures/maintext/empirical_training.pdf}
    \caption{Example on neural network not learning the designated ground truth features in the dataset. Designed ground truth features are both objects in the center and on the edge. Even though the model can achieve $100\%$ accuracy, our test shows that the model only learns to use designed features at the corner and ignore the central ground truth features (more detail in Appendix~\ref{sec:appendix:trained_nn_failure}). 
    % When providing the model with features in the image center, the model fails to predict correctly.
    }
    \label{fig:trained_nn}
\end{figure}

\begin{definition}\label{def_rashomon_effect}
Rashomon effect \citep{Breiman2001rashomon} (multiplicity of equally good models): There exist many models under the same hypothesis class that can achieve equally good accuracy but use different information for inference.
\end{definition}

Rashomon effect states that it is generally invalid to assume that a model with $100\%$ accuracy on a dataset $\mathcal{D}$ learns the true labeling process. In reality, depending on the data distribution, we can have trained models that learn to ignore some features that are relevant to the labels. Moreover, the model can learn other associations (e.g. use corners to classify a square). 
Specifically, neural networks tend to be over-parametrized for their learning tasks, hence making it harder to learn the true labeling function \citep{ba2014deep,frankle2018the}. We provide empirical evidence for trained neural networks ignoring designed features (detailed setting in Appendix~\ref{sec:appendix:trained_nn_failure}). The result in Figure~\ref{fig:trained_nn} shows a neural network, which achieves $100\%$ training accuracy, but learned to solely use partial ground truth features designed for the dataset (objects at the edge). 
Our analysis and examples in this section suggest that a model that learns to always perform correctly on the dataset is still not guaranteed to learn the intended ground truth features in the data. \emph{Therefore, we manually program the neural networks}.

By explicitly designing the data and the neural network according to specific properties, we can enable correct identifications of ground truth features in our synthetic setting. The ground truth features can then be used for evaluating feature attribution methods. 
One reasonable approach is to calculate precision and recall. However, since attribution maps usually have continuous pixel values, we adjust the metrics accordingly. Given an set of features $\mathcal{F}$ indexed by the index set $\mathcal{J} = \{j \in \mathbb{N}^{+} | 1 \leq j \leq |\mathcal{F}| \}$, let $a_j$ be the attribution value of the $j^{th}$ feature, and $g_j$ be the ground truth value of the $j^{th}$ feature, the (soft) precision is calculated as $\precision(\mathcal{F}) = \sum_{j \in \mathcal{J}}|a_j \cdot g_j|/\sum_{j \in \mathcal{J}}|a_j|$, while the recall is defined as $\recall(\mathcal{F}) = \sum_{j \in \mathcal{J}}|a_j \cdot g_j|/\sum_{j \in \mathcal{J}}|g_j|$. We normalize the attribution maps to $[-1, 1]$ to constrain the recall within the range of $[0, 1]$, as the ground truth masks are binary. Given the precision and recall, we can easily calculate the \Fone-score as well.

%----------END SUBSECTION----------%
\section{Design of data and neural network} \label{sec:method:design}
In this section, we provide a brief overview of the design of two synthetic evaluation settings designed to be representative of various evaluation scenarios. The two evaluation settings complement each other and differ in terms of model structure, tasks to be learned, and input data type.

%----------END SUBSUBSECTION----------%
\paragraph{Single-color-modulo}

Given monochromatic images as input, we manually program a synthetic neural network to count the number of white pixels in the image (the Accumulator) and output the modulo $N$ of the total pixel count (the Modulo), where the divisor $N$ is a predefined number.
%
The design of these images consists of multiple pixel patches of arbitrary shape within a constant background (reference value). 
%
The Accumulator and Modulo programs have \emph{properties} tailored toward evaluating feature attributions:
%
\begin{proposition}\label{def:sensitivity}
\textbf{(Sensitivity property)} 
The addition/removal of \textbf{any} ground truth pixel to/from the background affects the output of the neural network.
% A any ground truth feature with a non-ground truth feature affects the neural network output. 
\end{proposition}


\begin{proposition}\label{def:symmetry}
\textbf{(Symmetry property)} 
The addition/removal of any ground truth pixel to/from the background \textbf{equally} affects the output of the neural network.
% Replace any ground truth feature with a non-ground truth feature has an equal effect on the network output.
\end{proposition}


% \begin{definition}\label{def:completeness}
% \textbf{(Completeness)}: The number of pixels removed is equivalent to the output difference (with a linear coefficient for the Modulo program).
% \end{definition}

The Sensitivity property implies that \emph{every} ground truth (white) pixel is relevant to the neural network output, as the addition/removal of any ground truth (white) pixel to/from the background (black) affects their count. The symmetry property implies that every ground truth (white) pixel has \emph{equal} relevance to the output of the neural network. In our model design, the addition/removal of any ground truth (white) pixel to/from the background (black) equally affects the count of white pixels. Since we know each and every feature is equally relevant, we can use this ground truth relevance and compare it with feature attribution explanations (using metrics in Section~\ref{sec:method:transparent_env}). In fact, these properties are aligned with the sensitivity and symmetry feature attribution axioms ~\citep{ManyShapleySundararajan2020,sundararajan2017axiomatic,lundberg2017unified}, which axiomatically define the relevance of a feature.

% Consequently, we can infer that all white pixels (in any possible configuration) contribute to the decision-making process of the model, hence satisfying the \emph{Sensitivity} axiom \cite{lundberg2017unified,sundararajan2017axiomatic,ManyShapleySundararajan2020}.
% Furthermore, the removal of any white pixel causes the same output change in the model, thus also fulfilling the \emph{Symmetry} axiom. Therefore, for this task, our designed single-output neural network is aligned with the designed ground truth features, which are all white pixels, according to definitions. 
% %
% Moreover, the choice of modulo program leads to a classification task, as the output for any monochromatic image is bounded between $0$ and $K-1$. The property is needed as most feature attribution methods are proposed for classification models.
% Second, randomly generated images can yield a uniform distribution of output classes, eliminating any class imbalance issue. 

To develop a neural network model that can perform this task, we design a model that consists of two components. The first component is a Convolutional Neural Network (CNN) tasked with counting the total number of white pixels in the input image. This CNN accumulation module can be initialized with either uniform or non-uniform weights. 
To initialize this CNN with uniform weights, we can simply set all weights of CNN kernels to $1$. We further elaborate on the initialization of non-uniform weights in Appendix~\ref{sec:appendix:accumulator}. The second part of the model is a multilayer perceptron (MLP) designed to perform the modulo operation. 
We formally define the modulo module using functions. We first design a neural structure that can identify a specific integer number. For integer input, this structure can be defined as 
% \begin{equation}
%     I_N(x) = \relu(
%     \relu(\relu(x-N+1) - \relu(x-N))
%     -
%     \relu(\relu(x-N) - \relu(x-N-1))
%     ).
% \end{equation}
% \begin{equation}
%     \begin{aligned}
%         I_N(x) &= \relu(I_{N, +}(x) - I_{N, -}(x)) \\
%         \text{where } I_{N, +}(x) &= \relu(\relu(x-N+1) - \relu(x-N)), \\
%         \text{and } I_{N, -}(x) &= \relu(\relu(x-N) - \relu(x-N-1)). \\
%     \end{aligned}
% \end{equation}
\begin{equation}\label{eq:identify_number}
    \begin{aligned}
        I_N(x) &= \relu(I_{>N-1}(x) - I_{>N}(x)) \\
        \text{where } I_{>i}(x) &= \relu(\relu(x-i) - \relu(x-i-1)).
    \end{aligned}
\end{equation}
% $I_N(x) = \relu(
% \relu(\relu(x-N+1) - \relu(x-N))
% -
% \relu(\relu(x-N) - \relu(x-N-1))
% )$. 
We design $I_{>i}(x)$ such that $I_{>i}(x) = 1$ for all $x \in \{x \in \mathbb{N}|x > i\}$, otherwise $I_{>i}(x) = 0$. Furthermore, $I_N(x)$ ensures that $I_N(N) = 1$ and $\forall x \in \{x \in \mathbb{N}|x\neq N\}, I_N(x) = 0$. We leverage the number identification module $I_N(x)$ to further build up the neural modulo module. The first layer of the module is $f_1(x) = \relu(x, x-N, x-2N, ..., x-\lceil\frac{U}{N}\rceil N)$, where $U$ represents the maximal input value that the module can process, which can be scaled according to available computation resources. Note that $f_1$ produces a vector output. The second layer is defined as $f_2(\vec{x}) = \relu(x_0 - x_1, x_1 - x_2, ...)$. Thus, we would have $f_2(f_1(x)) = (N, N, ..., x  \mod  N, 0, ..., 0)$ after propagating through the first two layers. 
At this stage, our output only comprises three possible numbers: $N$, $x \mod N$, and $0$. Next, we eliminate the number $N$ in the output vector. This is accomplished by applying $f_3(\vec{x}) = \relu(x_0, I_N(x_0), x_1, I_N(x_1), ...)$, and $f_4(\vec{x}) = \relu(x_0 - N x_1, x_2 - N x_3, ...)$. Hence, we have $f_4(f_3(f_2(f_1(x)))) = (0, 0, ..., x  \mod  N, 0, ...)$. 
Lastly, we have one layer $f_5(\vec{x}) = \relu(\sum_{i=0}x_i)$ to accumulate the output vector. Therefore, as shown in Figure~\ref{fig:comp_graph}, we can obtain the modulo calculation with 
\begin{equation}
    f_{\text{modulo}, N}(x) = f_5(f_4(f_3(f_2(f_1(x))))) = x\mod N. 
\end{equation}
The complexity of the MLP model ensures that the synthetic model poses a moderate challenge for attribution methods. Further details regarding the dataset generation and model initialization can be found in Appendix~\ref{sec:appendix:number_check}, Appendix~\ref{sec:appendix:modulo}, and Appendix~\ref{sec:appendix:exp_black_white_bezier_dataset_generation}.
%----------END SUBSUBSECTION----------%
\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\columnwidth]{figures/maintext/comp_graph.pdf}
    \caption{Example computational graph of our designed neural network modules. Blue boxes symbolize neurons, with their respective computations indicated within the box. ReLU activation is applied after each neuron, which is omitted in the figure. The left example shows a neural network of identifying number $5$. The middle example shows the computation of modulo $5$ given input $8$, where the neural network is capable of calculating modulo $5$ for any number between $0$ and $100$. The right example shows a simple color detector for detecting RGB value $(255, 127, 0)$. }
    \label{fig:comp_graph}
\end{figure}
\paragraph{Multi-color-sum}
The other setting is designed to resemble real image classification tasks but with simplified features. 
The dataset comprises color images, each containing $N_C$ patches of uniquely colored foreground objects and a distinct background color that is consistent across images, resulting in $N_C + 1$ colors in every image. The images are input to the model in RGB format. By treating each foreground color as a class, we formulate a multi-class task to predict the dominant color in an image. The designed classification model outputs softmax scores using logits for $N_C$ classes, where the logit of each class corresponds to the sum of pixels of the respective color. The design of the model and the dataset also follow the properties in Proposition~\ref{def:sensitivity} and ~\ref{def:symmetry} as the output of each color detector is directly connected to the Accumulator module. Hence, we can infer that all colored pixels are relevant features. The addition of softmax on the Accumulator output makes pixels of colors other than the target negatively contribute to the output of the target color (after softmax). Thus the ground truth will have both positively and negatively contributing features, enabling us to evaluate whether an attribution method is able to discern between positive and negative contributions.

% Nevertheless, for this model, only an increase in the target output score contributes positively to the decision. Hence, we define pixels of the target color as positive ground truth features, while pixels of other colors that are not the background color are negative ground truth features, as they cause the target output score to decrease.

The design criterion for the model in this setting is more complex. We aim to create a model capable of accurately performing the task while also exhibiting unpredictable behavior when given OOD inputs. The model in this setting has three components. The first component is a CNN color detector responsible for detecting target colors and simulating OOD effects (detailed implementation in Appendix~\ref{sec:appendix:color_detector}). Its output has dimensions of $(N_C + N_R) \times H \times W$, where $N_C$ denotes the number of target classes and $N_R$ denotes the number of redundant channels. For the first $N_C$ channels, the $i^{th}$ output map is the activation of the $i^{th}$ target color. We briefly explain how to implement color detection in neural networks. Given a color to be detected that is in RGB format $(R, G, B)$, where $R$, $G$, and $B$ are integers within $[0, 255]$. For a pixel with intensity $(r, g, b)$, the color detection mechanism shown in Figure~\ref{fig:comp_graph} can be expressed as:
\begin{equation}
    C(r, g, b) = \relu(I_R(r) + I_G(g) + I_B(b) - 2).
\end{equation}
Here, the number identification functions $I_R$, $I_G$, and $I_B$ each detect a predefined component of an RGB value and are implemented as shown in Equation~\ref{eq:identify_number}. Hence, we have $C(r, g, b) = 1$ for $r=R, g=G,b=B$, and $C(r, g, b) = 0$ otherwise. 
The remaining $N_R$ redundant channels activate on any other colors not among the $N_C + 1$ colors defined in our dataset. Specifically, if any pixel has a color that is neither a target color nor the background color, all $N_R$ redundant channels will activate at the position of this pixel. 
The activation mechanism of redundant channels is implemented as 
\begin{equation}
    R(r, g, b) = \relu( - \sum C_i(r, g, b) + 1). 
\end{equation}
Consequently, $R(r ,g ,b) = 1$ if all $C_i(r,g,b) = 0$, and $R(r ,g ,b) = 1$ if $C_i(r,g,b) = 1$ for any $i$.
Following the color detector, we have a CNN module that accumulates activation of the first $N_C$ channels, respectively. The remaining $N_R$ redundant channels have random connections to the input of this CNN module. 
Therefore, the CNN accumulation module will have unexpected outputs if the input images contain any OOD colors. Lastly, we have an MLP that performs identity mapping, as the output of the CNN module already provides the logits of each target color for normal inputs. 
The rationale behind adding an identity MLP module is to preserve the conventional model architecture in image classification, where a model is typically designed as a CNN followed by an MLP head.

% \todo{fit in the text. }We briefly explain how to implement color detection in neural networks. Given a color to be detected that is in RGB format $(R, G, B)$, where $R$, $G$, and $B$ are integers within $[0, 255]$. For a pixel with intensity $(r, g, b)$, the color detection mechanism can be expressed as:
% \begin{equation}
%     C(r, g, b) = \relu(I_R(r) + I_G(g) + I_B(b) - 2).
% \end{equation}
% Here, the number identification functions $I_R$, $I_G$, and $I_B$ each detect predefined RGB values. Hence, we have $C(r, g, b) = 1$ for $r=R, g=G,b=B$, and $C(r, g, b) = 0$ otherwise. For a color detector that can detect $N_C$ colors, a redundant channel is implemented as 
% \begin{equation}
%     R(r, g, b) = \relu( - \sum_i^{N_{C}} C_i(r, g, b) + 1). 
% \end{equation}
% Consequently, the redundant channel is activated for any color not pre-defined by the color detector.
In multi-class classification, signed ground truth information is available, outlining the positive and negative contributions of features to the target class. To assess attribution methods with signed ground truth, we separately compute the precision, recall, and \Fone-score of the positive and negative portions of the attribution maps using their corresponding ground truth masks. Furthermore, we evaluate the entire attribution map using an unsigned union of both positive and negative ground truths: the \emph{overall ground truth}. This evaluation takes into consideration all features that contribute to decision-making, ignoring attribution value signs.

